KOFFVQA: An Objectively Evaluated Free-form VQA Benchmark for Large Vision-Language Models in the Korean Language

The recent emergence of Large Vision-Language Models(VLMs) has resulted in a variety of different benchmarks for evaluating such models. Despite this, we observe that most existing evaluation methods suffer from the fact that they either require the model to choose from pre-determined responses, sacrificing open-endedness, or evaluate responses using a judge model, resulting in subjective and unreliable evaluation. In addition, we observe a lack of benchmarks for VLMs in the Korean language, which are necessary as a separate metric from more common English language benchmarks, as the performance of generative language models can differ significantly based on the language being used. Therefore, we present KOFFVQA, a general-purpose free-form visual question answering benchmark in the Korean language for the evaluation of VLMs. Our benchmark consists of 275 carefully crafted questions each paired with an image and grading criteria covering 10 different aspects of VLM performance. The grading criteria eliminate the problem of unreliability by allowing the judge model to grade each response based on a pre-determined set of rules. By defining the evaluation criteria in an objective manner, even a small open-source model can be used to evaluate models on our benchmark reliably. In addition to evaluating a large number of existing VLMs on our benchmark, we also experimentally verify that our method of using pre-existing grading criteria for evaluation is much more reliable than existing methods. Our evaluation code is available at https://github.com/maum-ai/KOFFVQA

==> tables/1_amount.tex <==
\begin{table}[t]
\centering
\begin{tabular}{lc}
\hline
Subcategory                   & Count \\ \hline
Object Attributes             & 60    \\
Relationship                  & 30    \\
Recognition                   & 10    \\
Recognition-KO                & 10    \\
KO-OCR                        & 20    \\
Commonsense Reasoning         & 45    \\
Document Understanding        & 30    \\
Table Understanding           & 30    \\
Graph and Chart Understanding & 30    \\
Hallucination and Robustness  & 10    \\ \hline
\end{tabular}
\caption{The number of questions in each subcategory.}
\label{tab:amount}
\end{table}
